Satori: Towards Proactive AR Assistant with Belief-Desire-Intention User Modeling

Augmented Reality (AR) assistance is increasingly used for supporting users with physical tasks like assembly and cooking. However, most systems rely on reactive responses triggered by user input, overlooking rich contextual and user-specific information. To address this, we present Satori, a novel AR system that proactively guides users by modeling both -- their mental states and environmental contexts. Satori integrates the Belief-Desire-Intention (BDI) framework with the state-of-the-art multi-modal large language model (LLM) to deliver contextually appropriate guidance. Our system is designed based on two formative studies involving twelve experts. We evaluated the system with a sixteen within-subject study and found that Satori matches the performance of designer-created Wizard-of-Oz (WoZ) systems, without manual configurations or heuristics, thereby improving generalizability, reusability, and expanding the potential of AR assistance.

==> tables/action.tex <==
\begin{table}[]

\begin{tabular}{ccccc}
\toprule

Dataset & \multicolumn{2}{c}{GTEA}                      & \multicolumn{2}{c}{Our Dataset}               \\ \cmidrule(lr){2-3}\cmidrule(lr){4-5}
Task   & Action Recognition & Desired Task Recognition & Action Recognition & Desired Task Recognition \\ \hline
Li et al.~\cite{li2015delving}        & 62.10               & N/A                      & N/A                & N/A                      \\
Satori  & 79.50               & 100.00                      & 85.00                  & 100.00                     \\
\bottomrule
% \bottomrule
\end{tabular}
\caption{
\revision{Table showing the results for the desired task and action recognition. We evaluated Satori on the GTEA dataset~\cite{li2015delving} and our dataset over the top model on GTEA's leaderboard. } }
\label{tab:desire-task-prediction}
\end{table}



% \begin{table}[ht]
% \centering
% \begin{tabular}{lcc}
% \toprule
%  & GTEA (Accuracy \%) & Our Dataset (Accuracy \%) \\ 
% \midrule
% Intention Recognition & 79.5 & \textbf{85.0} \\
% Desire Prediction     & 100.0  & \textbf{100.0} \\
% Belief Prediction     & N/A  & TBD \\ %59.72 temporari, waiting for final dataset
% Modality Prediction   & N/A  & N/A \\
% \end{tabular}
% \end{table}


==> tables/streams.tex <==
\begin{table*}[!htbp]
    \centering

\begin{tabular}{|l|p{6cm}|l|}

\hline
Stream                   & Description                                                                                                                   & \multicolumn{1}{c|}{Data Format}    \\ \hline
main                     & The stream which contains the frames sent by HoloLens 2 headset                                                               & \multicolumn{1}{c|}{Image Bytes}    \\ \hline
processed\_main          & The stream which contains the frames processed by an image recognition module to filter out the related frames                & \multicolumn{1}{c}{Image Bytes}    \\ \hline
guidance                 & The stream used to store the generated guidance result                                                                        & \multicolumn{1}{c|}{JSON}           \\ \hline
assistant:images         & The stream used to store the generated image assistance.                                                                      & \multicolumn{1}{c|}{Protobuf Bytes} \\ \hline
intent:belief            & The stream used to store the inferred belief state.                                                                           & JSON                                \\ \hline
intent:desire            & The stream used to store the inferred desire state                                                                            & JSON                                \\ \hline
intent:task\_plan        & The stream used to store the task plan consisting the desired task plan and action checkpoints generated by the task plan LLM & JSON                                \\ \hline
intent:task:checkpoints  & The stream used to store the inferred states of the action checkpoints                                                        & JSON                                \\ \hline
intent:task:step:nex     & The stream used to store the inferred next intended action.                                                                   & JSON                                \\ \hline
intent:task:step:current & The stream used to store the inferred next intended action.                                                                   & JSON                                \\ \hline
feedback                 & The stream used to store the user' feedback.                                                                                  & JSON                                \\ \hline
\end{tabular}
\caption{The stream list used in the system. We list the stream names, corresponding descriptions, and data formats in the table. The names in the open-sourced code may be slightly different from the names in the development build.}
\label{tab:streams}
\end{table*}

==> tables/sus_former.tex <==
\begin{table}[]
    \centering
    

\begin{tabular}{lrl}
\toprule
 Question   &   Mean & 95\% Confidence Interval   \\
\midrule
 Q1      &   5.25 & 4.42 - 6.00               \\
 Q2      &   5.5  & 4.83 - 6.08               \\
 Q3      &   5.5  & 4.83 - 6.08               \\
 Q4      &   4.83 & 4.25 - 5.42               \\
 Q5      &   5    & 4.00 - 5.83               \\
 Q6      &   4.83 & 4.08 - 5.50               \\
 Q7      &   5.75 & 5.08 - 6.25               \\
 Q8      &   5.5  & 4.83 - 6.08               \\
 Q9      &   4.83 & 4.00 - 5.58               \\
\bottomrule
\end{tabular}
\caption{User ratings on the system usability using a seven-point Likert scale. The mean values and intervals computed through bootstrapping are presented in the table.}
\label{tab:sus_former}

\end{table}

==> tables/sus_legacy.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lccc}
\hline
Question & Condition & 95\% CI & $p$-value & $p$-value Non-Inferiority \\
\hline
I can easily comprehend the content via the text/audio/image guidance & KST & [5.25, 6.50] & \cellcolor{white}0.099 & \cellcolor{red!30}0.001 \\
 & WoZ & [6.00, 6.75] & & \\
\hline
The guidance's content is helpful in completion the task & KST & [5.50, 6.50] & \cellcolor{white}0.094 & \cellcolor{red!30}0.000 \\
 & WoZ & [5.75, 6.75] & & \\
\hline
I think the guidance appear at the right moment & KST & [5.00, 6.25] & \cellcolor{white}0.090 & \cellcolor{red!30}0.000 \\
 & WoZ & [5.88, 6.50] & & \\
\hline
I found that the guidance accurately reflects my task intentions. & KST & [5.62, 6.50] & \cellcolor{red!30}0.016 & \cellcolor{red!30}0.000 \\
 & WoZ & [6.00, 7.00] & & \\
\hline
The guidance appears at a adequate location & KST & [5.25, 6.25] & \cellcolor{red!30}0.032 & \cellcolor{red!30}0.000 \\
 & WoZ & [5.88, 6.75] & & \\
\hline
I am able to complete my work quickly using this system & KST & [5.25, 6.50] & \cellcolor{white}0.273 & \cellcolor{red!30}0.001 \\
 & WoZ & [5.50, 6.50] & & \\
\hline
It was easy to learn to use this system.  & KST & [5.75, 7.00] & \cellcolor{white}0.179 & \cellcolor{red!30}0.000 \\
 & WoZ & [6.00, 7.00] & & \\
\hline
how engaged I am using the system? & KST & [5.50, 6.38] & \cellcolor{white}0.145 & \cellcolor{red!30}0.001 \\
 & WoZ & [6.00, 6.50] & & \\
\hline
The system's guidance matches the context & KST & [5.62, 7.00] & \cellcolor{white}0.357 & \cellcolor{red!30}0.000 \\
 & WoZ & [5.88, 6.75] & & \\
\hline
Overall, the system's guidance frequency is suitable.  & KST & [5.75, 6.50] & \cellcolor{white}0.156 & \cellcolor{red!30}0.001 \\
 & WoZ & [5.75, 6.75] & & \\
\hline
Overall, I think the system can be beneficial in my everyday life. & KST & [5.25, 6.25] & \cellcolor{white}0.277 & \cellcolor{red!30}0.002 \\
 & WoZ & [5.50, 6.50] & & \\
\hline
\end{tabular}
\caption{Results for NASA TLX Questions and Non-Inferiority Tests}
\end{table}


==> tables/tlx_backup.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{p{5cm}ccccccc}
\hline
\multirow{2}{*}{Question} & \multirow{2}{*}{Condition}  & \multirow{2}{*}{Mean}  & \multirow{2}{*}{95\% CI}  & \multicolumn{2}{c}{Vanilla} &  \multicolumn{2}{c}{Non-Inferiority}  \\
& & & & W &$p$-value & W & $p$-value \\
\hline
\multirow{2}{5cm}{Mental Demand} & Satori & 34.06 & [17.50, 43.81] & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} \\
 & WoZ & 33.12 & [16.25, 50.00] & \multirow{-2}{*}{\cellcolor{white}60.500}  & \multirow{-2}{*}{\cellcolor{white}0.744}  & \multirow{-2}{*}{\cellcolor{white}78.000}  &\multirow{-2}{*}{\cellcolor{white}0.316}  \\
\hline
\multirow{2}{5cm}{Physical Demand} & Satori & 32.34 & [11.25, 50.00] & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} \\
 & WoZ & 30.47 & [10.00, 43.75] & \multirow{-2}{*}{\cellcolor{white}55.000}  & \multirow{-2}{*}{\cellcolor{white}0.776}  & \multirow{-2}{*}{\cellcolor{white}80.000}  &\multirow{-2}{*}{\cellcolor{white}0.281}  \\
\hline
\multirow{2}{5cm}{Temporal Demand} & Satori & 28.52 & [21.25, 37.50] & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} \\
 & WoZ & 26.41 & [15.00, 32.50] & \multirow{-2}{*}{\cellcolor{white}46.000}  & \multirow{-2}{*}{\cellcolor{white}0.274}  & \multirow{-2}{*}{\cellcolor{white}65.000}  &\multirow{-2}{*}{\cellcolor{white}0.388}  \\
\hline
\multirow{2}{5cm}{Performance} & Satori & 16.17 & [7.50, 21.25] & \cellcolor{white} & \cellcolor{white} & \cellcolor{lightgreen} & \cellcolor{lightgreen} \\
 & WoZ & 17.27 & [7.50, 20.00] & \multirow{-2}{*}{\cellcolor{white}44.000}  & \multirow{-2}{*}{\cellcolor{white}0.593}  & \multirow{-2}{*}{\cellcolor{lightgreen}95.500}  &\multirow{-2}{*}{\cellcolor{lightgreen}0.022}  \\
\hline
\multirow{2}{5cm}{Effort} & Satori & 28.20 & [17.50, 37.50] & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} & \cellcolor{white} \\
 & WoZ & 26.02 & [15.00, 36.25] & \multirow{-2}{*}{\cellcolor{white}52.500}  & \multirow{-2}{*}{\cellcolor{white}0.464}  & \multirow{-2}{*}{\cellcolor{white}58.500}  &\multirow{-2}{*}{\cellcolor{white}0.353}  \\
\hline
\multirow{2}{5cm}{Frustration} & Satori & 19.84 & [10.00, 28.75] & \cellcolor{white} & \cellcolor{white} & \cellcolor{lightgreen} & \cellcolor{lightgreen} \\
 & WoZ & 26.95 & [11.25, 34.38] & \multirow{-2}{*}{\cellcolor{white}41.500}  & \multirow{-2}{*}{\cellcolor{white}0.175}  & \multirow{-2}{*}{\cellcolor{lightgreen}126.000}  &\multirow{-2}{*}{\cellcolor{lightgreen}0.001}  \\
\hline
\end{tabular}
% \caption{Results for NASA TLX Questions and Non-Inferiority Tests}
% \end{table}
% \label{tab:tlx}
\caption{Results for NASA TLX Questions and Non-Inferiority Tests. This table shows the mean scores and 95\% confidence intervals (CI) for Satori and WoZ systems across six dimensions: Mental Demand, Physical Demand, Temporal Demand, Performance, Effort, and Frustration. The Vanilla Wilcoxon signed-rank test results and non-inferiority tests (highlighted in green) indicate whether the Satori system performs comparably or better than the WoZ system in terms of cognitive load.}
\label{tab:tlx}
\end{table}

